Online Unsupervised Learning of Visual Representations and Categories

Real world learning scenarios involve a nonstationary distribution of classes with sequential dependencies among the samples, in contrast to the standard machine learning formulation of drawing samples independently from a fixed, typically uniform distribution. Furthermore, real world interactions demand learning on-the-fly from few or no class labels. In this work, we propose an unsupervised model that simultaneously performs online visual representation learning and few-shot learning of new categories without relying on any class labels. Our model is a prototype-based memory network with a control component that determines when to form a new class prototype. We formulate it as an online mixture model, where components are created with only a single new example, and assignments do not have to be balanced, which permits an approximation to natural imbalanced distributions from uncurated raw data. Learning includes a contrastive loss that encourages different views of the same image to be assigned to the same prototype. The result is a mechanism that forms categorical representations of objects in nonstationary environments. Experiments show that our method can learn from an online stream of visual input data and its learned representations are significantly better at category recognition compared to state-of-the-art self-supervised learning methods.

==> sections/abstract_oneline.tex <==
Real world learning scenarios involve a nonstationary distribution of classes with sequential dependencies among the samples, in contrast to the standard machine learning formulation of drawing samples independently from a fixed, typically uniform distribution. Furthermore, real world interactions demand learning on-the-fly from few or no class labels. In this work, we propose an unsupervised model that simultaneously performs online visual representation learning and few-shot learning of new categories without relying on any class labels. Our model is a prototype-based memory network with a control component that determines when to form a new class prototype. We formulate it as an online Gaussian mixture model, where components are created online with only a single new example, and assignments do not have to be balanced, which permits an approximation to natural imbalanced distributions from uncurated raw data. Learning includes a contrastive loss that encourages different views of the same image to be assigned to the same prototype. The result is a mechanism that forms categorical representations of objects in nonstationary environments. Experiments show that our method can learn from an online stream of visual input data and is significantly better at category recognition compared to state-of-the-art self-supervised learning methods.

==> sections/metrics.tex <==
% !TEX root = ../main.tex
\section{Evaluation metrics details}

\paragraph{Rand index:} The rand index is a simpler way of computing the similarity between two data clusterings\footnote{\url{https://en.wikipedia.org/wiki/Rand_index}}, by comparing pairwise labels. It is defined as:
\begin{align}
    RI = \frac{a+b}{a+b+c+d} = \frac{a+b}{\binom{n}{2}},
\end{align}
where $n$ is the total number of elements,
\begin{itemize}
    \item $a$ is the number of pairs of elements that are in the {\it same} subsets in $U$ and the {\it same} subsets in $V$;
    \item $b$ is the number of pairs of elements that are in {\it different} subsets in $U$ and {\it different} subsets in $V$;
    \item $c$ is the number of pairs of elements that are in the {\it same} subsets in $U$ and {\it different} subsets in $V$;
    \item $d$ is the number of pairs of elements that are in {\it different} subsets in $U$ and the {\it same} subsets in $V$.
\end{itemize}
The adjusted Rand index subtracts a baseline of the expected value by random chance by fixing the number and size of clusters:
\begin{align}
    ARI = \frac{\sum_{ij} \binom{n_{ij}}{2} - \left[ \sum_i \binom{a_i}{2} \sum_j \binom{b_j}{2} \right] \Big/ \binom{n}{2}}{\frac{1}{2}\left[ \sum_i \binom{a_i}{2} + \sum_j \binom{b_j}{2}\right] - \left[ \sum_i \binom{a_i}{2} \sum_j \binom{b_j}{2} \right] \Big/ \binom{n}{2}}
\end{align}
\paragraph{Completeness:}
The completeness score is to measure how often the items from the same class are assigned to the same cluster.
\begin{align}
    c = 1 - \frac{H(K|C)}{H(K)},
\end{align}
where $H(K|C)$ is the conditional entropy of the cluster assignments given the classes, and $H(K)$ is the entropy of the cluster assignments.

\paragraph{Homogeneity:}
The homogeneity score is to measure how often one cluster contain only one class.
\begin{align}
    h = 1 - \frac{H(C|K)}{H(C)},
\end{align}
where $H(C|K)$ is the conditional entropy of the classes given the cluster assignments, and $H(C)$ is the entropy of the classes.

\paragraph{Adjusted mutual information (AMI):} We consider the adjusted mutual information score. The mutual information between two random variable $X, Y$ is defined as
\begin{align}
    I(X;Y) = \sum_{y\in Y} \sum_{x \in X} p(x,y) \log \left( \frac{p(x,y)}{p(x)p(y)} \right).
\end{align}
Suppose we have two clustering $U = \{U_i\}$ and $V = \{V_j\}$, and $U_i$ and $V_j$ are set of example IDs, and $N$ is the total number of examples. $U$ and $V$ can be viewed as discrete probability distribution over cluster IDs.
\begin{align}
    p(x=i) & = \frac{\lvert U_i \rvert}{N} = \frac{a_i}{N}, \\ 
    p(y=j) & = \frac{\lvert V_j \rvert}{N} = \frac{b_j}{N}, \\ 
    p(x=i, y=j) & = \frac{ \lvert U_i \cap V_j \rvert}{N} = \frac{n_{ij}}{N}.
\end{align}
Therefore, we can define the mutual information score between $U$ and $V$:
\begin{align}
    MI(U, V) &= \sum_{i=1}^{\lvert U \rvert} \sum_{j=1}^{\lvert V \rvert} \frac{ \lvert U_i \cap V_j\rvert }{N} \log \left( \frac{N \lvert U_i \cap V_j\rvert }{\lvert U_i \rvert \lvert V_j \rvert} \right) \\
    &= \sum_{i=1}^R \sum_{j=1}^C \frac{n_{ij}}{N} \log \left( \frac{N n_{ij}}{a_i b_j} \right).
\end{align}
The adjusted MI score\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.metrics.adjusted_mutual_info_score.html}} normalizes the range between 0 and 1, and subtracts the random chance. The goal here is to make two random clustering return 0, and two identical clustering return 1.
\begin{align}
    AMI(U, V) &= \frac{MI(U, V) - \mathbb{E}[MI(U,V)]}{\frac{1}{2}(H(U) + H(V))  - \mathbb{E}[MI(U,V)]},
\end{align}
where $H(\cdot)$ denotes the entropy function, and $\mathbb{E}[MI(U,V)]$ is the expected mutual information by chance \footnote{\url{https://en.wikipedia.org/wiki/Adjusted_mutual_information}}:
\begin{align}
    \mathbb{E}[MI(U,V)] = \sum_{i=1}^R \sum_{j=1}^C \sum_{n=s_{ij}}^{t_{ij}} \frac{n}{N} \log\left( \frac{N n}{a_i b_j} \right) \frac{a_i!b_j!(N-a_i)!(N-b_j)!}{N!n!(a_i-n)!(b_j-n)!(N-a_i-b_j+n)!},
\end{align}
where $s_{i,j}=\max(1, a_i + b_j -N)$, and $t_{ij}=\min(a_i, b_j)$.

\paragraph{Average precision (AP)}
